Strong Copyright Protection for Language Models via Adaptive Model Fusion

The risk of language models unintentionally reproducing copyrighted material from their training data has led to the development of various protective measures. In this paper, we propose model fusion as an effective solution to safeguard against copyright infringement. In particular, we introduce Copyright-Protecting Fusion (CP-Fuse), an algorithm that adaptively combines language models to minimize the reproduction of protected materials. CP-Fuse is inspired by the recently proposed Near-Access Free (NAF) framework and additionally incorporates a desirable balancing property that we demonstrate prevents the reproduction of memorized training data. Our results show that CP-Fuse significantly reduces the memorization of copyrighted content while maintaining high-quality text and code generation. Furthermore, we demonstrate how CP-Fuse can be integrated with other techniques for enhanced protection.

==> sections/conclusion.tex <==
\section{Conclusions}


==> sections/theory.tex <==


\section{Toy Model Example}
\label{sec:theory}
Complementary to our experimental analysis in Section~\ref{sec:experiments}, we present in this section a theoretically discussion on the copyright material leakage. Frameworks for guarantees on the worst-case copyright material leakage, similar to differential privacy, are still widely underdeveloped. With the k-NAF framework, \citet{vyas2023provable} presents a first attempt. However, their guarantees are strongly tied to standard sampling for generation and thus only to a limited extent meaningful when generating text using common greedy search based inference techniques. Moreover, their guarantees rely on quantities that are inherently difficult to estimate and interpret. Instead, in this paper we take a different approach by studying an idealized toy model that allows us to better understand the copyright protection mechnism implemented by our algorithm, as well as 
demonstrate how our algorithm proposed in Section~\ref{sec:algo} successfully overcome the limitations of the approaches proposed in \cite{vyas2023provable,li2024purifying} summarized in Section~\ref{sec:preliminaries}.




% % \subsection{Protection against greedy search strategies}
% As illustrated in Figure~bla in the Appendix, memorization of training samples causes the model trained on a dataset to return almost deterministic distributions when the prompt is sufficiently close to prompts used for training. As a result, greedy search inference algorithms likely output large sequences of copyright material. We now present a theoretical discussion on a highly simplified toy-example that  demonstrates how our algorithm in Section~\ref{sec:algo} prevents the reproduction of verbatim copyright protected material. 

\paragraph{Setting} We consider a situation where for a given prompt $x$, the first model $p^{(1)}$ strongly memorizes a copyright protected sequence $y^*$. Without loss of generality, we may assume that the protected sequence $y^*_{\leq T}= [\text{a}, \cdots, \text{a}]$ consists of all a. For simplicity, we assume that the sequence length is always exactly $T>0$, and we model the logitis of $p^{(1)}$ to be
\begin{equation}
    \forall t: p^{(1)}(y_t \vert y^*_{< t}) = \begin{cases}
        1-\delta &  y_t =\text{a}, \\
        \frac{\delta}{ m_t} &  y_t \in \Omega_t\setminus \{a\}
\\
        0 & \text{else}
    \end{cases}
\end{equation}
where $\Omega_t$ is a set of plausible tokens given $y_{<t}$ that contains $a$ of size $m_t+1 := \vert \Omega_t\vert $. For simplicity, we may assume that $\Omega_t = \Omega$ for all $t$, and thus $m_t = m$. 
By the \textit{separability of copyright material} assumption from Section~\ref{sec:preliminaries}, the model $p^{(2)}$ has never seen the copyright protected sequence $y^*_{\leq T}$ during training. We therefore model $   p^{(2)}$  by
\begin{equation}
    \forall t:\quad  p^{(2)}(y_t \vert y_{<t}, x) = \begin{cases}
        \alpha & y_t = a\\
       \frac{ \gamma}{K} & y_t \in S_t \\
       \frac{1-\gamma - \alpha}{\vert V\vert -K} &  \text{else}
    \end{cases}
\end{equation}
where $S \setminus \{a\} $ is a random subset of $V$ of size $K$ drawn uniformly at random.














 % memorization of training samples causes the model trained on a dataset to return almost deterministic distributions when the prompt is sufficiently close to prompts used for training. As a result, greedy search inference algorithms likely output large sequences of copyright material. We now present a theoretical discussion on a highly simplified toy-example that  demonstrates how our algorithm in Section~\ref{sec:algo} prevents the reproduction of verbatim copyright protected material. 

